Low Spin-Axis Variations of Circumbinary Planets

Having a massive moon has been considered as a primary mechanism for stabilized planetary obliquity, an example of which being our Earth. This is, however, not always consistent with the exoplanetary cases. This article details the discovery of an alternative mechanism, namely that planets orbiting around binary stars tend to have low spin-axis variations. This is because the large quadrupole potential of the stellar binary could speed up the planetary orbital precession, and detune the system out of secular spin-orbit resonances. Consequently, habitable zone planets around the stellar binaries in low inclination orbits hold higher potential for regular seasonal changes comparing to their single star analogues.

==> CBP obliquity_ArXiv/journal_macros.tex <==
\newcommand*\aap{A\&A}
\let\astap=\aap
\newcommand*\aapr{A\&A~Rev.}
\newcommand*\aaps{A\&AS}
\newcommand*\actaa{Acta Astron.}
\newcommand*\aj{AJ}
\newcommand*\ao{Appl.~Opt.}
\let\applopt\ao
\newcommand*\apj{ApJ}
\newcommand*\apjl{ApJ}
\let\apjlett\apjl
\newcommand*\apjs{ApJS}
\let\apjsupp\apjs
\newcommand*\aplett{Astrophys.~Lett.}
\newcommand*\apspr{Astrophys.~Space~Phys.~Res.}
\newcommand*\apss{Ap\&SS}
\newcommand*\araa{ARA\&A}
\newcommand*\azh{AZh}
\newcommand*\baas{BAAS}
\newcommand*\bac{Bull. astr. Inst. Czechosl.}
\newcommand*\bain{Bull.~Astron.~Inst.~Netherlands}
\newcommand*\caa{Chinese Astron. Astrophys.}
\newcommand*\cjaa{Chinese J. Astron. Astrophys.}
\newcommand*\fcp{Fund.~Cosmic~Phys.}
\newcommand*\gca{Geochim.~Cosmochim.~Acta}
\newcommand*\grl{Geophys.~Res.~Lett.}
\newcommand*\iaucirc{IAU~Circ.}
\newcommand*\icarus{Icarus}
\newcommand*\jcap{J. Cosmology Astropart. Phys.}
\newcommand*\jcp{J.~Chem.~Phys.}
\newcommand*\jgr{J.~Geophys.~Res.}
\newcommand*\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
\newcommand*\jrasc{JRASC}
\newcommand*\memras{MmRAS}
\newcommand*\memsai{Mem.~Soc.~Astron.~Italiana}
\newcommand*\mnras{MNRAS}
\newcommand*\na{New A}
\newcommand*\nar{New A Rev.}
\newcommand*\nat{Nature}
\newcommand*\nphysa{Nucl.~Phys.~A}
\newcommand*\pasa{PASA}
\newcommand*\pasj{PASJ}
\newcommand*\pasp{PASP}
\newcommand*\physrep{Phys.~Rep.}
\newcommand*\physscr{Phys.~Scr}
\newcommand*\planss{Planet.~Space~Sci.}
\newcommand*\pra{Phys.~Rev.~A}
\newcommand*\prb{Phys.~Rev.~B}
\newcommand*\prc{Phys.~Rev.~C}
\newcommand*\prd{Phys.~Rev.~D}
\newcommand*\pre{Phys.~Rev.~E}
\newcommand*\prl{Phys.~Rev.~Lett.}
\newcommand*\procspie{Proc.~SPIE}
\newcommand*\qjras{QJRAS}
\newcommand*\rmxaa{Rev. Mexicana Astron. Astrofis.}
\newcommand*\skytel{S\&T}
\newcommand*\solphys{Sol.~Phys.}
\newcommand*\sovast{Soviet~Ast.}
\newcommand*\ssr{Space~Sci.~Rev.}
\newcommand*\zap{ZAp}

==> CBP obliquity_ArXiv/macros.tex <==
% Warning unsolved, \overset might be used wrongly
\newcommand{\copyrightnotice}{\enlargethispage{24pt}
\let\thefootnote\relax\footnote{\copyright\ 2015 Christopher Heil}}

\newcommand{\EQ}{\; = \;}
\newcommand{\NE}{\; \ne\;}
\newcommand{\GE}{\; \ge\;}
\newcommand{\GT}{\; > \;}
\newcommand{\LE}{\; \le\;}
\newcommand{\LT}{\; < \;}
\newcommand{\TO}{\; \to\;}
\newcommand{\MAPSTO}{\; \mapsto\;}
\newcommand{\Capp}{\, \cap\,}
\newcommand{\CAP}{\; \cap\;}
\newcommand{\Cupp}{\, \cup\,}
\newcommand{\CUP}{\; \cup\;}
\newcommand{\MONOTONE}{\; \monotone\;}
\newcommand{\DECREASE}{\; \decrease\;}
\newcommand{\APPROX}{\; \approx\;}
\newcommand{\EQUIVNORM}{\; \asymp\;}
\newcommand{\Iff}{\; \iff\;}
\newcommand{\IFF}{\quad \iff\quad}
\newcommand{\Implies}{\; \implies\;}
\newcommand{\IMPLIES}{\quad \implies\quad}
\newcommand{\IN}{\; \in\;}
\newcommand{\NOTIN}{\; \not\in\;}
\newcommand{\NOTTO}{\; \notto\;}
\newcommand{\NOTIMPLIES}{\quad \Longrightarrow\hskip -14 pt / \hskip 4 pt \quad}
\newcommand{\oneway}{\quad
 \genfrac{}{}{0pt}{}{\implies}{\Longleftarrow\hskip -14 pt / \hskip 4 pt} \quad}
\newcommand{\SUBSET}{\; \subseteq\;}
\newcommand{\SUBSETEQ}{\; \subseteq\;}
\newcommand{\SUBSETNEQ}{\; \subsetneq\;}
\newcommand{\SUPSETEQ}{\; \supseteq\;}
\newcommand{\CONG}{\; \cong\;}
\newcommand{\plus}{\; + \;}
\newcommand{\minus}{\;-\;}
\newcommand{\completeimplies}{\underset{\text{if~$X$ is complete}} \IMPLIES}

%\newcommand{\svee}{{\scriptscriptstyle{\vee}}}
\newcommand{\svee}{{\hbox{\raise.4ex \hbox{${\scriptscriptstyle{\vee}}$}}}}
\newcommand{\swedge}{{\hbox{\raise.4ex \hbox{${\scriptscriptstyle{\wedge}}$}}}}
\newcommand{\sveeexp}{\svee\tinyback}
\newcommand{\swedgeexp}{\swedge\tinyback}
\newcommand{\swedgehat}[1]{\overset{\scriptscriptstyle{\wedge}}{#1}}
\newcommand{\sveecheck}[1]{\overset{\scriptscriptstyle{\vee}}{#1}}

\newcommand{\Ac}{{\mathcal{A}}}
\newcommand{\AC}{\mathrm{AC}}
\newcommand{\avg}{\textup{Avg}}
\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\betabar}{\overline{\beta}}
\newcommand{\Bc}{{\mathcal{B}}}
%\newcommand{\ball}{{\mathrm{Ball}}}
%\newcommand{\Ball}{{\mathrm{Ball}}}
\newcommand{\ball}{D}
\newcommand{\littleback}{\hskip -0.6 true pt}
\newcommand{\tinyback}{\hskip -1 true pt}
\newcommand{\bigback}{\hskip -1.5 true pt}
\newcommand{\bigabs}[1]{\bigl|#1\bigr|}
\newcommand{\Bigabs}[1]{\Bigl|#1\Bigr|}
\newcommand{\biggabs}[1]{\biggl|#1\biggr|}
\newcommand{\bigbracket}[1]{\bigl[#1\bigr]}
\newcommand{\Bigbracket}[1]{\Bigl[#1\Bigr]}
\newcommand{\biggbracket}[1]{\biggl[#1\biggr]}
\newcommand{\borel}{{\Bc_\sigma}}
\newcommand{\BV}{\mathrm{BV}}
% \newcommand{\C}{\mathbb{C}}
\newcommand{\Cc}{{\mathcal{C}}}
\newcommand{\chat}{\widehat{c}\tinyspace}
\newcommand{\chatprime}{\chat^{\,\prime}}
%\newcommand{\ccheck}{\sveecheck{c}}
\newcommand{\ccheck}{\overset{\scriptscriptstyle{\hskip 1.5 pt \vee}}{c}}
\newcommand{\ccard}{{\mathfrak{c}}}
\newcommand{\card}{\textup{card}}
\newcommand{\ceiling}[1]{\lceil#1 \rceil}
\newcommand{\veecheck}[1]{\overset\vee#1}
\newcommand{\CHI}{\hbox{\raise.4ex \hbox{$\chi$}}}
\newcommand{\CHIA}{\CHI_{\hskip -0.7 true pt A}}
\newcommand{\CHIhat}{\widehat{\CHI}}
\newcommand{\CHINhat}
    {\CHI_{\!N} \hskip -10.5pt \widehat{\phantom{\CHI}} \hskip 3 pt}
\newcommand{\CHINcheck}
    {\overset{\scriptscriptstyle{\hskip 4.0 pt \vee}} \CHI_{\!N}}
\newcommand{\CHIOmegacheck}
    {\overset{\scriptscriptstyle{\hskip 2.5 pt \vee}} \CHI_{\!\varOmega}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\clspan}{{\overline{\mbox{\rm span}}}}
\newcommand{\codim}{{\textup{codim}}}
\newcommand{\Col}{\textup{Col}}
\newcommand{\comp}{{\mathrm{C}}}
\newcommand{\medcap}{\operatornamewithlimits{\textstyle\bigcap}}
\newcommand{\medcup}{\operatornamewithlimits{\textstyle\bigcup}}
\newcommand{\smallcup}{\operatornamewithlimits{\scriptstyle\bigcup}}
\newcommand{\scap}{\hbox{\raise.25ex
\hbox{${\operatornamewithlimits{\scriptstyle\bigcap}}$}}}
\newcommand{\scup}{\hbox{\raise.25ex
\hbox{${\operatornamewithlimits{\scriptstyle\bigcup}}$}}}
\newcommand{\ddx}{\frac{d}{dx}}
\newcommand{\Dc}{{\mathcal{D}}}
\newcommand{\decrease}{\searrow}
\newcommand{\deltahat}{\widehat{\delta}}
\newcommand{\deltacheck}
  {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} \delta}
\newcommand{\di}{\displaystyle}
\newcommand{\diam}{{\textup{diam}}}
\newcommand{\dist}{{\textup{dist}}}
\newcommand{\domain}{{\textup{domain}}}
\newcommand{\tE}{{\widetilde{E}}}
\newcommand{\Ec}{{\mathcal{E}}}
\newcommand{\Emptyset}{\varnothing}
\newcommand{\bigenumspace}{\vglue-4 pt}
\newcommand{\enumspace}{\vglue-3 pt}
\newcommand{\smallenumspace}{\vglue-2 pt}
\newcommand{\eps}{\varepsilon}
%\newcommand{\esssup}{\mathop{\text{\rm ess \, sup}}}
\newcommand{\esssup}{\operatornamewithlimits{{\textup{ess\tinyspace\ sup}}}}
\newcommand{\bigeval}[1]{{\bigl. #1 \bigr|}}
\newcommand{\Bigeval}[1]{{\Bigl. #1 \Bigr|}}
\newcommand{\biggeval}[1]{{\biggl. #1 \biggr|}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fc}{{\mathcal{F}}}
\newcommand{\tFc}{{\widetilde{\mathcal{F}}}}
\newcommand{\Fcheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} F}
\newcommand{\fcheck}{\fveecheck}
\newcommand{\fhat}{\widehat{f}}
%\newcommand{\fhat}{\overset {\scriptscriptstyle{\hskip 4 pt\wedge}} f}
\newcommand{\fwedgehat}
    {\overset{\lower.6ex \hbox{${\scriptscriptstyle{\hskip 3 pt\wedge}}$}} f}
\newcommand{\fveecheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} f}
\newcommand{\fkcheck}
   {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 1 pt\vee}}$}} {f_k}}
%\newcommand{\fhatcheck}{\bigparen{\fwedgehat\tinyspace}^{\bigback\svee}}
\newcommand{\fhatcheck}{\bigparen{\fhat\biggerspace}^{\bigback\svee}}
\newcommand{\fcheckhat}{\bigparen{\fveecheck\tinyspace}^{\tinyback\swedge}}
\newcommand{\fhatprime}{\fhat^{\hskip 3pt\raiseprime}}
\newcommand{\raiseprime}{\hbox{\raise.3ex \hbox{${\scriptstyle{\prime}}$}}}
%\newcommand{\fhatprime}{\fhat^{\tinyspace\prime}}
\newcommand{\fprimehat}{\widehat{f'\littlespace}}
\newcommand{\flambdahat}
    {f_\lambda\hskip -8.5pt \widehat{\phantom{f}} \hskip 3 pt}
\newcommand{\tf}{\widetilde{f} \rule{0pt}{10.6pt}}
\newcommand{\tfh}{\widetilde{f}_{\hskip -0.2 true pt h}}
\newcommand{\tfhn}{\widetilde{f}_{\hskip -0.2 true pt h_n}}
%\newcommand{\tfh} {f_h \hskip -8pt \widetilde{\phantom{f}} \hskip 2 pt}
\newcommand{\fbar}{\bar{f} \rule{0pt}{10.4pt}}
%\newcommand{\tfhat}{\widehat{\widetilde{f}}}
\newcommand{\tfhat} {\widetilde{f}
    \hskip -4.5pt \widehat{\phantom{\widetilde{f}}} \hskip -1.5 pt}
\newcommand{\fkhat} {f_k \hskip -8pt \widehat{\phantom{f}} \hskip 2 pt}
\newcommand{\fmhat} {f_m \hskip -10pt \widehat{\phantom{f}} \hskip 4 pt}
\newcommand{\fnhat} {f_n \hskip -8pt \widehat{\phantom{f}} \hskip 2 pt}
\newcommand{\floor}[1]{\lfloor\tinyback#1 \tinyback\rfloor}
\newcommand{\Gc}{{\mathcal{G}}}
\newcommand{\Gcheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} G}
\newcommand{\ghat}{\widehat{g}}
%\newcommand{\gcheck}{\check{g}}
\newcommand{\ghatcheck}{\bigparen{\ghat\biggerspace}^{\bigback\svee}}
%\newcommand{\ghatcheck}{g^{\swedge\svee}}
\newcommand{\gcheck}{\gveecheck}
\newcommand{\gveecheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} g}
\newcommand{\gcheckhat}{\bigparen{\gveecheck\tinyspace}^{\tinyback\swedge}}
\newcommand{\gprimehat}{\tinyback\widehat{\,g'\,}\tinyback}
\newcommand{\glambdahat}
    {g_\lambda\hskip -8.5pt \widehat{\phantom{g}} \hskip 3 pt}
\newcommand{\glambdaprime}{g_\lambda^{\;\prime}}
\newcommand{\gnhat}{\widehat{g_n}}
\newcommand{\tg}{\widetilde{g}}
%\newcommand{\tgh}{\widetilde{g}_{\hskip -0.1 true pt h}}
\newcommand{\tgh} {g_h \hskip -8pt \widetilde{\phantom{g}} \hskip 2 pt}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\graph}{{\textup{graph}}}
\newcommand{\wedgehat}[1]{\overset\wedge#1}
\newcommand{\tH}{\widetilde{H}}
\newcommand{\hhat}{\widehat{h}}
\newcommand{\Hhat}{\widehat{H}}
\newcommand{\Hc}{{\mathcal{H}}}
\newcommand{\Hf}{H \hskip -0.7 true pt f}
\newcommand{\hcheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} h}
\newcommand{\hnhat} {h_n \hskip -10pt \widehat{\phantom{h}} \hskip 4 pt}
%\newcommand{\Th}{\widetilde{h}}
\newcommand{\Herm}{{\text{H}}}
\newcommand{\HS}{{\text{HS}}}
\newcommand{\Imag}{\textup{Im}}
\newcommand{\ip}[2]{\langle#1,#2\rangle}
\newcommand{\bigip}[2]{\bigl\langle#1, \, #2 \bigr\rangle}
\newcommand{\Bigip}[2]{\Bigl\langle#1, \, #2 \Bigr\rangle}
\newcommand{\biggip}[2]{\biggl\langle#1, \, #2 \biggr\rangle}
\newcommand{\boxip}[2]{[#1,#2]}
\newcommand{\itema}{{\item{\textup{(a)}}}}
\newcommand{\itemb}{\item{\textup{(b)}}}
\newcommand{\Khat}{\widehat{K}}
\newcommand{\Kcheck}
  {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} K}
\newcommand{\khat}{\widehat{k}}
\newcommand{\kNhat}{\widehat{k_N}}
\newcommand{\tk}{\widetilde{k}}
\newcommand{\klambdahat}
    {k_\lambda\hskip -8.5pt \widehat{\phantom{k}} \hskip 3 pt}
%\newcommand{\klambdahat}{\overset {\tinyspace\wedge} {k_\lambda}}
\newcommand{\klambdatilde}
    {k_\lambda\hskip -8.5pt \widetilde{\phantom{k}} \hskip 3 pt
     \rule{0pt}{10.6pt}}
\newcommand{\kntilde}{k_n \hskip -8.5pt \widetilde{\phantom{k}} \hskip 3 pt}
\newcommand{\Lc}{{\mathcal{L}}}
\newcommand{\Lip}{\textup{Lip}}
\newcommand{\loc}{{\mathrm{loc}}}
\newcommand{\Lpt}{\widetilde{L^p}}
\newcommand{\Liminf}{\operatornamewithlimits{{\textup{lim\tinyspace\ inf}}}}
\newcommand{\Limsup}{\operatornamewithlimits{{\textup{lim\littlespace\ sup}}}}
\newcommand{\textmax}{{\mathrm{max}}}
\newcommand{\textmin}{{\mathrm{min}}}
\newcommand{\Mbar}{\overline{M}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\Mf}{M \hskip -0.7 true pt f}
\newcommand{\bmat}[1]{\left[\begin{array}{rrrrrrr} #1 \end{array}\right]}
\newcommand{\bmatf}[1]{\left[\begin{array}{ccccccc} #1 \end{array}\right]}
\newcommand{\bmatcen}[1]{\left[\begin{array}{ccccccc} #1 \end{array}\right]}
\newcommand{\smallbmat}[1]{\left[\smallmatrix#1 \endsmallmatrix\right]}
\newcommand{\measure}{\operatorname{\overset\ m \to}} 
\newcommand{\metric}{\mathrm{d}}
\newcommand{\monotone}{\nearrow}
\newcommand{\tmonotone}{\tinyback\nearrow\tinyback}
\newcommand{\tmu}{\widetilde{\mu}}
\newcommand{\mucheck}{\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 2 pt\vee}}$}} \mu}
\newcommand{\muhat}{\widehat{\mu}}
\newcommand{\mubar}{\overline{\mu}}
\newcommand{\nuhat}{\widehat{\nu}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\notimplies}{{\Longrightarrow\hskip -14 pt / \hskip 4 pt}}
\newcommand{\notto}{{\hskip 2 pt \rightarrow\hskip -10 pt / \hskip 6 pt}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\bignorm}[1]{\bigl\|#1\bigr\|}
\newcommand{\Bignorm}[1]{\Bigl\|#1\Bigr\|}
\newcommand{\biggnorm}[1]{\biggl\|#1\biggr\|}
\newcommand{\tnu}{\widetilde{\nu}}
\newcommand{\Oc}{{\mathcal{O}}}
\newcommand{\medoplus}{\operatornamewithlimits{\textstyle\bigoplus}}
\newcommand{\Omegab}{\mathbf{\varOmega}}
\newcommand{\osc}{{\textup{osc}}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Pbb}{{\mathbf{P}}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\pv}{{\textup{pv}}}
\newcommand{\bigparen}[1]{\bigl(#1\bigr)}
\newcommand{\Bigparen}[1]{\Bigl(#1\Bigr)}
\newcommand{\biggparen}[1]{\biggl(#1\biggr)}
\newcommand{\Biggparen}[1]{\Biggl(#1\Biggr)}
\newcommand{\parensize}[1]{\left(#1\right)}
\newcommand{\phat}{\widehat{p}\tinyspace}
\newcommand{\phihat}{\widehat{\phi}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\varphihat}{\widehat{\varphi}}
\newcommand{\tvarphi}{\widetilde{\varphi} \rule{0pt}{9.8pt} }
\newcommand{\varphixihat}
    {\varphi_{\xi} \hskip -9pt \widehat{\phantom{\varphi}} \hskip 2.5 pt}
\newcommand{\varphixikhat}
    {\varphi_{\xi_k} \hskip -9pt \widehat{\phantom{\varphi}} \hskip 2.5 pt}
\newcommand{\varphixitilde}
    {\varphi_{\xi} \hskip -9pt \widetilde{\phantom{\varphi}} \hskip 2.5 pt}
\newcommand{\varphionehat}
    {\varphi_{1} \hskip -9.5pt \widehat{\phantom{\varphi}} \hskip 1.5 pt}
\newcommand{\varphimhat}
    {\varphi_m \hskip -9pt \widehat{\phantom{\varphi}} \hskip 2.5 pt}
\newcommand{\varphinhat}
    {\varphi_n \hskip -10.0pt \widehat{\phantom{\varphi}} \hskip 2.5 pt}
\newcommand{\varphicheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 1 pt\vee}}$}}
              \varphi}
\newcommand{\psihat}{\widehat{\psi}}
\newcommand{\psixihat}
    {\psi_{\xi} \hskip -9pt \widehat{\phantom{\psi}} \hskip 2.5 pt}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Qc}{{\mathcal{Q}}}
\newcommand{\tQ}{{\widetilde{Q}}}
\newcommand{\qeddef}{{\quad $\diamondsuit$}}
%\newcommand{\qeddef}{{$\ \hfill \diamondsuit$}}
\newcommand{\qeddeff}{{\qquad \diamondsuit}}
\newcommand{\qeddefff}{{\quad \diamondsuit}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rc}{{\mathcal{R}}}
\newcommand{\Rhat}{\widehat{\R}}
%\newcommand{\Rbar}{{\bar{R}}}
\newcommand{\Rbar}
  {{\overset{\hskip -0.9 pt \lower\ 1.5pt \hbox{{\rule{6.7pt}{0.45pt}}}} \R}}
\newcommand{\subRbar}
   {{\overset{\hskip -0.8 pt \lower\ 1.5pt \hbox{{\rule{4.5pt}{0.5pt}}}} \R}}
\newcommand{\Real}{\textup{\text{Re}}}
\newcommand{\range}{{\textup{range}}}
\newcommand{\clrange}{{\overline{\mbox{\rm range}}}}
\newcommand{\rank}{{\textup{rank}}}
\newcommand{\row}{{\text{---}}}
%\newcommand{\shah}{\operatorname{\text{\cyr Sh}}}
\newcommand{\Sc}{{\mathcal{S}}}
\newcommand{\bS}{\bar{S}}
\newcommand{\tS}{\widetilde{S}}
%\newcommand{\SNa}{S_N^{\hskip 0.5 pt \hbox{\small a}}}
\newcommand{\SNa}{S_N^{\hskip 0.5 pt
  \hbox{\raise.3ex \hbox{\small\textup{a}}}}}
\newcommand{\SNaa}[1]{S_#1^{\hskip 0.5 pt
  \hbox{\raise.3ex \hbox{\small\textup{a}}}}}
%\newcommand{\SNa}{S_N^{\hskip 0.5 pt a}}
\newcommand{\SNo}{S_N^{\hskip 0.5 pt
  \hbox{\raise.3ex \hbox{\small\textup{o}}}}}
%\newcommand{\SNo}{S_N^{\hskip 0.5 pt \hbox{o}}}
%\newcommand{\SNo}{S_N^{\hskip 1 pt o}}
\newcommand{\SNt}{S_N^{\hskip 0.5 pt
  \hbox{\raise.3ex \hbox{\small\textup{t}}}}}
\newcommand{\SN}{S_N \hskip -0.6 pt}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\bigset}[1]{\bigl\{#1\bigr\}}
\newcommand{\Bigset}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\biggset}[1]{\biggl\{#1\biggr\}}
\newcommand{\setsize}[1]{\left\{#1\right\}}
\newcommand{\Sigmabar}{\overline{\varSigma}}
\newcommand{\sgn}{{\mathrm{sgn}}}
\newcommand{\sign}{{\mathrm{sign}}}
\newcommand{\sinc}{{\mathrm{sinc}}}
\newcommand{\sskip}[1]{{\vspace{0.#1 true in}}}
\newcommand{\smallestskip}{{\vspace{1 pt}}}
\newcommand{\smallerskip}{{\vspace{2 pt}}}
\newcommand{\tiniestspace}{\hskip 0.6 pt}
\newcommand{\tinierspace}{\hskip 0.8 pt}
\newcommand{\tinyspace}{\hskip 1 pt}
\newcommand{\littlespace}{\hskip 1.2 pt}
\newcommand{\bigspace}{\hskip 1.5 pt}
\newcommand{\biggerspace}{\hskip 2 pt}
%\newcommand{\solution}{\vskip 0.1 true in \noindent
%\underbar{Solution} \newline \indent}
%\newcommand{\solutionf}{\vskip 0.1 true in \noindent \underbar{Solution}}
%\newcommand{\solutionp}{\noindent \underbar{Solution} \newline \indent}
%\newcommand{\booksolution}{\noindent{\it Solution}. }
\newcommand{\Span}{\mathrm{span}}
\newcommand{\spectrum}{\mathrm{Sp}}
%\newcommand{\subset}{\subseteq}
\newcommand{\supp}{{\textup{supp}}}
\newcommand{\trans}{{\text{T}}}
\newcommand{\T}{{\mathbb{T}}}
\newcommand{\Tb}{{\mathbf{T}}}
\newcommand{\Tc}{{\mathcal{T}}}
\newcommand{\Tt}{{\textup{T}}}
%\newcommand{\Top}{{\mathcal{T}}}
\newcommand{\takeaway}{\hskip 0.8 pt \backslash\hskip 0.8 pt}
\newcommand{\tensor}{\otimes}
\newcommand{\textm}{{\mathrm{m}}}
\newcommand{\thetahat}{\widehat{\theta}}
\newcommand{\thetalambdahat}{\widehat{\theta_\lambda}}
\newcommand{\thetaMhat}{\widehat{\theta_M}}
\newcommand{\transpose}{{\mathrm{T}}}
\newcommand{\trace}{{\mathrm{trace}}}
\newcommand{\spaceback}{\hskip -1.2 true pt}
\newcommand{\tripnorm}[1]{{{|}\spaceback{|}\spaceback{|} #1
                           {|}\spaceback{|}\spaceback{|}}}
%\newcommand{\tripnorm}[1]{{{|}\!{|}\!{|} #1 {|}\!{|}\!{|}}}
\newcommand{\quadnorm}[1]{{{|}\spaceback{|}\spaceback{|}\spaceback{|} #1
                           {|}\spaceback{|}\spaceback{|}\spaceback{|}}}
\newcommand{\Uc}{{\mathcal{U}}}
\newcommand{\uni}{{\mathrm{u}}}
\newcommand{\vhat}{\widehat{v}}
\newcommand{\vlambdahat}
    {v_\lambda\hskip -8.5pt \widehat{\phantom{v}} \hskip 2.5 pt}
\newcommand{\itsyvertrule}{\rule{0pt}{5.2pt}}
\newcommand{\tiniestvertrule}{\rule{0pt}{6.8pt}}
\newcommand{\tiniervertrule}{\rule{0pt}{8.2pt}}
\newcommand{\tinyvertrule}{\rule{0pt}{8.8pt}}
\newcommand{\smallvertrule}{\rule{0pt}{9.5pt}}
\newcommand{\smallervertrule}{\rule{0pt}{9.6pt}}
\newcommand{\medvertrule}{\rule{0pt}{9.8pt}}
\newcommand{\meddervertrule}{\rule{0pt}{10.1pt}}
\newcommand{\vertrule}{\rule{0pt}{10.4pt}}
\newcommand{\bigvertrule}{\rule{0pt}{10.8pt}}
\newcommand{\biggervertrule}{\rule{0pt}{11.8pt}}
\newcommand{\Bigvertrule}{\rule{0pt}{13.2pt}}
%\newcommand{\vertspace}{\phantom{\widehat{\Sigma}\!}}
\newcommand{\vertspace}{\phantom{\Bigparen{X}\!}}
\newcommand{\bigvertspace}{\phantom{\Biggparen{X}}\!\!}
\newcommand{\vol}{{\mathrm{vol}}}
\newcommand{\what}{\widehat{w}}
%\newcommand{\wcheck}{\sveecheck{w}}
\newcommand{\wcheck}{\overset{\scriptscriptstyle{\hskip 1.5 pt \vee}} w}
\newcommand{\Wc}{{\mathcal{W}}}
\newcommand{\Wchat}{\widehat{\Wc}}
%\newcommand{\What}{\swedgehat{W}}
\newcommand{\What}{W \hskip -9.0pt \widehat{\phantom{T}} \hskip 1.5 pt}
\newcommand{\Wcheck}{\sveecheck{W}}
\newcommand{\wlambdahat}
    {w_\lambda\hskip -10pt \widehat{\phantom{w}} \hskip 2.5 pt}
\newcommand{\WsubN}{W_{\!N}\tinyback}
\newcommand{\WN}{W_{\tinyback\ N}}
\newcommand{\weak}{\operatorname{\overset{w}{\to}}} 
\newcommand{\notweak}{{\weak\hskip -9 pt / \hskip 8 pt}}
\newcommand{\weakstar}{\operatorname{\overset{w\text{*}}{\longrightarrow}}} 
%\newcommand{\weakstar}{\operatorname{\overset w\text{*} \to \to}} 
\newcommand{\Weak}{\textup{Weak-}}
\newcommand{\widecheck}[1]{\overset{\vee}{#1}}
\newcommand{\xhat}{\widehat{x}}
\newcommand{\xnhat} {x_n \hskip -9pt \widehat{\phantom{x}} \hskip 3 pt}
\newcommand{\tx}{\widetilde{x}}
\newcommand{\tX}{\widetilde{X}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zc}{{\mathcal{Z}}}
\newcommand{\zeroveecheck}
    {\overset{\lower.4ex \hbox{${\scriptscriptstyle{\hskip 0.5 pt\vee}}$}} 0}

%\newcommand{\indexspacer}{\rule{0pt}{10.6pt}}
%\newcommand{\indexspacer}{}

\newcommand{\indexspaced}{\rule{0pt}{11.8pt}}
%\newcommand{\bigindexspacer}{\rule{0pt}{13.9pt}}
\newcommand{\bigindexspacer}{\rule{0pt}{13.9pt}}

\hyphenation{Bun-ya-kow-ski}
\hyphenation{spatial}

\newcommand{\solution}{\vspace{0.1 true in} \noindent
\underbar{Solution} \newline \indent}
\newcommand{\solutionf}{\vspace{0.1 true in} \noindent \underbar{Solution}}
\newcommand{\solutionp}{\noindent \underbar{Solution} \newline \indent}
\newcommand{\booksolution}{\noindent{\it Solution}. }

\newcommand{\dashint}{\mathop{\,\rlap{--}\!\!\!\int}\nolimits}

==> journal_macros.tex <==
\newcommand*\aap{A\&A}
\let\astap=\aap
\newcommand*\aapr{A\&A~Rev.}
\newcommand*\aaps{A\&AS}
\newcommand*\actaa{Acta Astron.}
\newcommand*\aj{AJ}
\newcommand*\ao{Appl.~Opt.}
\let\applopt\ao
\newcommand*\apj{ApJ}
\newcommand*\apjl{ApJ}
\let\apjlett\apjl
\newcommand*\apjs{ApJS}
\let\apjsupp\apjs
\newcommand*\aplett{Astrophys.~Lett.}
\newcommand*\apspr{Astrophys.~Space~Phys.~Res.}
\newcommand*\apss{Ap\&SS}
\newcommand*\araa{ARA\&A}
\newcommand*\azh{AZh}
\newcommand*\baas{BAAS}
\newcommand*\bac{Bull. astr. Inst. Czechosl.}
\newcommand*\bain{Bull.~Astron.~Inst.~Netherlands}
\newcommand*\caa{Chinese Astron. Astrophys.}
\newcommand*\cjaa{Chinese J. Astron. Astrophys.}
\newcommand*\fcp{Fund.~Cosmic~Phys.}
\newcommand*\gca{Geochim.~Cosmochim.~Acta}
\newcommand*\grl{Geophys.~Res.~Lett.}
\newcommand*\iaucirc{IAU~Circ.}
\newcommand*\icarus{Icarus}
\newcommand*\jcap{J. Cosmology Astropart. Phys.}
\newcommand*\jcp{J.~Chem.~Phys.}
\newcommand*\jgr{J.~Geophys.~Res.}
\newcommand*\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}
\newcommand*\jrasc{JRASC}
\newcommand*\memras{MmRAS}
\newcommand*\memsai{Mem.~Soc.~Astron.~Italiana}
\newcommand*\mnras{MNRAS}
\newcommand*\na{New A}
\newcommand*\nar{New A Rev.}
\newcommand*\nat{Nature}
\newcommand*\nphysa{Nucl.~Phys.~A}
\newcommand*\pasa{PASA}
\newcommand*\pasj{PASJ}
\newcommand*\pasp{PASP}
\newcommand*\physrep{Phys.~Rep.}
\newcommand*\physscr{Phys.~Scr}
\newcommand*\planss{Planet.~Space~Sci.}
\newcommand*\pra{Phys.~Rev.~A}
\newcommand*\prb{Phys.~Rev.~B}
\newcommand*\prc{Phys.~Rev.~C}
\newcommand*\prd{Phys.~Rev.~D}
\newcommand*\pre{Phys.~Rev.~E}
\newcommand*\prl{Phys.~Rev.~Lett.}
\newcommand*\procspie{Proc.~SPIE}
\newcommand*\qjras{QJRAS}
\newcommand*\rmxaa{Rev. Mexicana Astron. Astrofis.}
\newcommand*\skytel{S\&T}
\newcommand*\solphys{Sol.~Phys.}
\newcommand*\sovast{Soviet~Ast.}
\newcommand*\ssr{Space~Sci.~Rev.}
\newcommand*\zap{ZAp}
